The Fast and the Private: Task-based Dataset Search

Modern dataset search platforms employ ML task-based utility metrics instead of relying on metadata-based keywords to comb through extensive dataset repositories. In this setup, requesters provide an initial dataset, and the platform identifies complementary datasets to augment (join or union) the requester's dataset such that the ML model (e.g., linear regression) performance is improved most. Although effective, current task-based data searches are stymied by (1) high latency which deters users, (2) privacy concerns for regulatory standards, and (3) low data quality which provides low utility. We introduce Mileena, a fast, private, and high-quality task-based dataset search platform. At its heart, Mileena is built on pre-computed semi-ring sketches for efficient ML training and evaluation. Based on semi-ring, we develop a novel Factorized Privacy Mechanism that makes the search differentially private and scales to arbitrary corpus sizes and numbers of requests without major quality degradation. We also demonstrate the early promise in using LLM-based agents for automatic data transformation and applying semi-rings to support causal discovery and treatment effect estimation.

==> sections/arch.tex <==
\section{Putting Everything Together}
\stitle{Solutions.} 
Current task-based data search platforms~\cite{santos2022sketch,chepurko2020arda,nargesian2022responsible,li2021data} follow the architecture illustrated in black in \Cref{fig:arch}. 
Offline, when providers upload raw datasets to {\it Data storage}, the platform computes minhashes for data discovery~\cite{castelo2021auctus,fernandez2018aurum}, and sketches to accelerate retraining~\cite{santos2022sketch,chepurko2020arda,nargesian2022responsible,kitana}. 
Online, the platform solves \Cref{searchprob} for each request  $(R_{train},R_{test},M)$.   First, {\it data discovery}~\cite{fernandez2018aurum,castelo2021auctus} uses the minhashes or sketches to return a set of candidate datasets. {\it Data search} then identifies a subset that maximizes task utility. The brute-force search evaluates all possible combinations and can be expensive due to retraining costs and the large set of combinations, so approaches use various heuristics and greedy algorithms~\cite{santos2022sketch,chepurko2020arda,li2021data}. 

==> sections/exp.tex <==
\section{Evaluation}

We evaluate \fdp on  NYC Open Data~\cite{nycopen} corpus of 329  datasets for an end-to-end dataset search.


\stitle{Data and Workload.} We construct a large data corpus of 329 NYC Open Data~\cite{nycopen} datasets.  We use  \textbf{Gender}~\cite{gender} dataset, which contains 2013-16 ELA data by grades and gender; check our paper for a more complete experiment results.


\subsection{AutoML Experiment}

\begin{figure}
    \centering
    \includegraphics[width=1.\columnwidth]{images/intro.pdf}
    \vspace*{-8mm}
    \caption{AutoML performance (testing $R2$) for $Gender$ dataset. The time budget is 10 minutes (dotted vertical line). \sys allocates $\sim3$ minutes for data augmentation using a corpus of 517 datasets with a proxy model and reaches $R2=\sim0.7$; \sys then sends the augmented dataset to AutoML and further improves $R2$ to $0.82$ with the remaining budget. Other baselines are either slow or have low $R2$.}
    \label{fig:moneyfig}
\end{figure}

\Cref{fig:moneyfig} summarizes our major results compared to prior data augmentation techniques (ARDA~\cite{chepurko2020arda}, Novelty~\cite{li2021data}); AutoML libraries (Auto-sklearn); and cloud AutoML services (Google's Vertex AI). Since augmentation techniques don't accept a time budget and return the augmented dataset, we run them to completion and then run Auto-sklearn to derive a model.
Both Auto-sklearn and Vertex AI only take the original training dataset as input, thereby neglecting the abundant augmentation opportunities that may be present in the data corpus.
We set Auto-sklearn's budget to 10 minutes and Vertex AI's budget to 1 hour (minimum allowed), and report $R2$ throughout the model search; Vertex AI doesn't enforce the budget.  



